Dexterous Non-Prehensile Manipulation for Ungraspable Object via Extrinsic Dexterity

Objects with large base areas become ungraspable when they exceed the end-effector's maximum aperture. Existing approaches address this limitation through extrinsic dexterity, which exploits environmental features for non-prehensile manipulation. While grippers have shown some success in this domain, dexterous hands offer superior flexibility and manipulation capabilities that enable richer environmental interactions, though they present greater control challenges. Here we present ExDex, a dexterous arm-hand system that leverages reinforcement learning to enable non-prehensile manipulation for grasping ungraspable objects. Our system learns two strategic manipulation sequences: relocating objects from table centers to edges for direct grasping, or to walls where extrinsic dexterity enables grasping through environmental interaction. We validate our approach through extensive experiments with dozens of diverse household objects, demonstrating both superior performance and generalization capabilities with novel objects. Furthermore, we successfully transfer the learned policies from simulation to a real-world robot system without additional training, further demonstrating its applicability in real-world scenarios. Project website: https://tangty11.github.io/ExDex/.

==> rebuttal_pics/DiffHeightObj.tex <==
\begin{figure}[!ht]
\centering

\includegraphics[width=0.7\linewidth]{rebuttal_pics/DiffHeightObj.png}
\vspace{-6pt}
\caption{Performance of objects with varying heights}
\label{fig:re_diff}
\vspace{-10pt}

\end{figure}

==> rebuttal_pics/Figure1.tex <==
\begin{figure}[!ht]
\centering

\includegraphics[width=1.0\linewidth]{rebuttal_pics/Figure1.pdf}
\vspace{-15pt}
\caption{(a-c): Comparison of \textit{ArmOnly}, \textit{Heuristic}, and \textit{Ours}. (d): Visualization of our tasks. (e-f): Unseen objects in simulation and real-world.}
\label{fig:re_figure1}
\vspace{-15pt}

\end{figure}

==> rebuttal_tabs/baseline.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
\caption{
   Quantitative Results of Baselines and Our Method. 
   % , and the necessities of different components of our method.
   }
\label{tab:rebuttal_baseline}
\centering
\setlength{\tabcolsep}{3pt}
\scriptsize
\begin{tabular}{l|cc|cc|cc|cc|cc|cc}

\toprule
 & \multicolumn{4}{c|}{Wall} & \multicolumn{4}{c|}{Edge} & \multicolumn{4}{c}{Left Edge}\\

\midrule
\multirow{2}{*}{Method}
 & \multicolumn{2}{c|}{Seen}
 & \multicolumn{2}{c|}{Unseen}
 & \multicolumn{2}{c|}{Seen}
 & \multicolumn{2}{c|}{Unseen}
 & \multicolumn{2}{c|}{Seen}
 & \multicolumn{2}{c}{Unseen}\\

 & TTE  & SR
 & TTE  & SR
 & TTE  & SR
 & TTE  & SR 
 & TTE  & SR
 & TTE  & SR 
 \\
\midrule
HACMAN 
& 42.46$\pm$0.00  & 39.09$\pm$0.00  & 0.65$\pm$0.00  
& 42.46$\pm$0.00  & 56.53$\pm$0.00  & 0.53$\pm$0.00  
& 28.17$\pm$0.00  & 22.60$\pm$0.00  & 0.87$\pm$0.00  
& 28.92$\pm$0.00  & 36.93$\pm$0.00  & 0.55$\pm$0.00  
\\
  
% Ungraspable~\cite{zhou2023learning} & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  \\

% MR：(reward ablation)去掉target reward
% ST：(reward ablation)去掉flag
% LargeFunnel：用movetp微调push，moverot微调wall/edge前
% JT：(joint training ablation)小模块joint training前

distill. 
& -  & -  & 0.0  
& -  & -  & 0.0  
& -  & -  & 0.06  
& -  & -  & 0.03  
\\

Fixed hand. 
& -  & -  & 0.0  
& -  & -  & 0.0  
& -  & -  & 0.0  
& -  & -  & 0.0  
\\

Heuristic. 
& -  & -  & 0.0  
& -  & -  & 0.0  
& -  & -  & 0.06  
& -  & -  & 0.03  
\\

w/o MR. 
& 0.22  & 4.28  & 0.78
& 0.46  & 16.05  & 0.05
& 3.42  & 44.19  & 0.72
& 3.41  & 4.95   & 0.40 
\\

w/o ST. 
& 0.22  & 4.28  & 0.78
& 0.46  & 16.05  & 0.05
& 3.42  & 44.19  & 0.72
& 3.41  & 4.95   & 0.40 
\\

% w/o CL. 
% & 0.28  & 2.33  & 0.79  
% & 0.22  & 4.16  & 0.55  
% & 3.40  & 2.40  & 0.95 
% & 3.48  & 34.10  & 0.71  
% \\

 w/o JF. 
& 0.28  & 2.33  & 0.79  
& 0.22  & 4.16  & 0.55  
& 3.40  & 2.40  & 0.95 
& 3.48  & 34.10  & 0.71  
\\

\textbf{Ours} 
& \textbf{0.20}  & \textbf{2.30}  & \textbf{0.73}  
& \textbf{0.21}  & \textbf{4.19}  & \textbf{0.55}  
& \textbf{3.68}  & \textbf{2.22}  & \textbf{0.99}  
& \textbf{3.61}  & \textbf{32.34}  & \textbf{0.75} 
\\%final
\bottomrule

\end{tabular}


\end{table*}

==> tabs/base_exp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
\caption{
   Quantitative Results of Baselines and Our Method. 
   % , and the necessities of different components of our method.
   }
\label{tab:base_exp}
\centering
\setlength{\tabcolsep}{8pt}
\small
\begin{tabular}{l|ccc|ccc|ccc|ccc}

\toprule
 & \multicolumn{6}{c|}{Wall} & \multicolumn{6}{c}{Edge}\\

\midrule
\multirow{2}{*}{Method}
 & \multicolumn{3}{c|}{Seen}
 & \multicolumn{3}{c|}{Unseen}
 & \multicolumn{3}{c|}{Seen}
 & \multicolumn{3}{c}{Unseen}\\

 & TTE & PTE & SR
 & TTE & PTE &SR
 & TTE & PTE &SR
 & TTE & PTE &SR 
 \\
\midrule
Random target 
& 42.46  & 39.09  & 0.65  
& 42.46  & 56.53  & 0.53  
& 28.17  & 22.60  & 0.87  
& 28.92  & 36.93  & 0.55  
\\
  
% Ungraspable~\cite{zhou2023learning} & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  \\

% MR：(reward ablation)去掉target reward
% ST：(reward ablation)去掉flag
% LargeFunnel：用movetp微调push，moverot微调wall/edge前
% JT：(joint training ablation)小模块joint training前

Ours w/o MR. 
& -  & -  & 0.0  
& -  & -  & 0.0  
& -  & -  & 0.0  
& -  & -  & 0.0  
\\

Ours w/o ST. 
& -  & -  & 0.0  
& -  & -  & 0.0  
& -  & -  & 0.06  
& -  & -  & 0.03  
\\

Ours w/o CL. 
& 0.22  & 4.28  & 0.78
& 0.46  & 16.05  & 0.05
& 3.42  & 44.19  & 0.72
& 3.41  & 4.95   & 0.40 
\\

Ours w/o JT. 
& 0.28  & 2.33  & 0.79  
& 0.22  & 4.16  & 0.55  
& 3.40  & 2.40  & 0.95 
& 3.48  & 34.10  & 0.71  
\\

\textbf{Ours} 
& \textbf{0.20}  & \textbf{2.30}  & \textbf{0.73}  
& \textbf{0.21}  & \textbf{4.19}  & \textbf{0.55}  
& \textbf{3.68}  & \textbf{2.22}  & \textbf{0.99}  
& \textbf{3.61}  & \textbf{32.34}  & \textbf{0.75} 
\\%final
\bottomrule

\end{tabular}


\end{table*}

==> tabs/base_exp_1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
\caption{
   Quantitative Results of Baselines and Our Method. 
   % , and the necessities of different components of our method.
   }
\label{tab:base_exp}
\centering
\setlength{\tabcolsep}{4pt}
\footnotesize
\begin{tabular}{l|cc|cc|cc|cc|cc|cc}

\toprule
 & \multicolumn{4}{c|}{Wall} & \multicolumn{4}{c|}{Front Edge} & \multicolumn{4}{c}{Left Edge}\\

\midrule
\multirow{2}{*}{Method}
 & \multicolumn{2}{c|}{Seen}
 & \multicolumn{2}{c|}{Unseen}
 & \multicolumn{2}{c|}{Seen}
 & \multicolumn{2}{c}{Unseen}
 & \multicolumn{2}{c|}{Seen}
 & \multicolumn{2}{c}{Unseen}\\

 & TTE & SR
 & TTE & SR
 & TTE & SR
 & TTE & SR 
 & TTE & SR
 & TTE & SR
 \\
\midrule
Random target 
& 30.87  & 0.45  
& 29.96  & 0.21  
& 3.74  & 0.69  
& 36.63  & 0.47  
& 3.74  & 0.69  
& 36.63  & 0.47  
\\
  
% Ungraspable~\cite{zhou2023learning} & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  \\

% MR：(reward ablation)去掉target reward
% ST：(reward ablation)去掉flag
% LargeFunnel：用movetp微调push，moverot微调wall/edge前
% JT：(joint training ablation)小模块joint training前

Ours w/o MR. 
& -  & 0.0  
& -  & 0.0  
& -  & 0.0  
& -  & 0.0  
& -  & 0.06  
& -  & 0.03 
\\

Ours w/o ST. 
& -  & 0.0  
& -  & 0.0  
& -  & 0.06  
& -  & 0.03  
& -  & 0.06  
& -  & 0.03 
\\

Ours w/o CL. 
& -  & 0.0  
& -  & 0.0  
& -  & 0.06  
& -  & 0.03 
& -  & 0.06  
& -  & 0.03 
\\

Ours w/o JT. 
& 0.28  & 2.33  & 0.79  
& 0.22  & 4.16  & 0.55  
& 3.40  & 2.40  & 0.95 
& 3.48  & 34.10  & 0.71  
& 2.35  & 3.73  & 0.87  
& 2.16  & 14.75  & 0.61 
\\

\textbf{Ours} 
& \textbf{0.20}  & \textbf{2.22}  & \textbf{0.73}  
& \textbf{0.21}  & \textbf{0.73}  & \textbf{0.55}  
& \textbf{3.68}  & \textbf{2.22}  & \textbf{0.99}  
& \textbf{3.61}  & \textbf{32.34}  & \textbf{0.75} 
& \textbf{2.14}  & \textbf{3.55}  & \textbf{0.94}  
& \textbf{2.20}  & \textbf{4.30}  & \textbf{0.68}
\\%final
\bottomrule

\end{tabular}


\end{table*}

==> tabs/base_exp_copy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
\caption{
   Quantitative Results of Baselines and Our Method. 
   % , and the necessities of different components of our method.
   }
\label{tab:base_exp}
\centering
\setlength{\tabcolsep}{4pt}
\footnotesize
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|ccc}

\toprule
 & \multicolumn{6}{c|}{Wall} & \multicolumn{6}{c|}{Front Edge} & \multicolumn{6}{c}{Left Edge}\\

\midrule
\multirow{2}{*}{Method}
 & \multicolumn{3}{c|}{Seen}
 & \multicolumn{3}{c|}{Unseen}
 & \multicolumn{3}{c|}{Seen}
 & \multicolumn{3}{c}{Unseen}
 & \multicolumn{3}{c|}{Seen}
 & \multicolumn{3}{c}{Unseen}\\

 & TTE & PTE & SR
 & TTE & PTE & SR
 & TTE & PTE & SR
 & TTE & PTE & SR 
 & TTE & PTE & SR
 & TTE & PTE & SR
 \\
\midrule
Random target 
& 30.87  & 26.89  & 0.45  
& 29.96  & 26.16  & 0.21  
& 3.74  & 3.49  & 0.69  
& 36.63  & 37.50  & 0.47  
& 3.74  & 3.49  & 0.69  
& 36.63  & 37.50  & 0.47  
\\
  
% Ungraspable~\cite{zhou2023learning} & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  & 0.  \\

% MR：(reward ablation)去掉target reward
% ST：(reward ablation)去掉flag
% LargeFunnel：用movetp微调push，moverot微调wall/edge前
% JT：(joint training ablation)小模块joint training前

Ours w/o MR. 
& - & - & 0.0  
& - & -  & 0.0  
& -  & -  & 0.0  
& -  & -  & 0.0  
& -  & -  & 0.06  
& -  & -  & 0.03 
\\

Ours w/o ST. 
& - & - & 0.0  
& - & -  & 0.0  
& -  & -  & 0.06  
& -  & -  & 0.03  
& -  & -  & 0.06  
& -  & -  & 0.03 
\\

Ours w/o LF. 
& - & - & 0.0  
& - & -  & 0.0  
& -  & -  & 0.06  
& -  & -  & 0.03 
& -  & -  & 0.06  
& -  & -  & 0.03 
\\

Ours w/o JT. 
& - & - & 0.0  
& - & -  & 0.0  
& -  & -  & 0.06  
& -  & -  & 0.03  
& -  & -  & 0.06  
& -  & -  & 0.03 
\\

\textbf{Ours} &\textbf{0.20}  & \textbf{2.27}  & \textbf{0.73}  
& \textbf{0.21}  & \textbf{4.20}  & \textbf{0.55}  
& \textbf{3.68}  & \textbf{2.29}  & \textbf{0.99}  
& \textbf{3.61}  & \textbf{24.64}  & \textbf{0.75} 
& \textbf{2.14}  & \textbf{3.59}  & \textbf{0.94}  
& \textbf{2.20}  & \textbf{11.29}  & \textbf{0.68}
\\%final
\bottomrule

\end{tabular}


\end{table*}

==> tabs/cross_emb.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[tb]
\caption{
   \textbf{Quantitative Results of Baselines, Ablations and Our Method in Different Tasks. }
   These results demonstrate the strong performance of our method over baselines and ablations.
   % , and the necessities of different components of our method.
   }
\begin{center}

\small
\setlength{\tabcolsep}{1.0mm}{
\begin{tabular}{c|cccc|cccc}

\hline
\textbf{Task} & \multicolumn{4}{c|}{\textbf{Edge}} & \multicolumn{4}{c}{\textbf{Table}}\\

\hline
\multirow{2}{*}{\textbf{Hand}}
 & \multicolumn{2}{c}{\textbf{Train}}
 & \multicolumn{2}{c|}{\textbf{Test}}
 & \multicolumn{2}{c}{\textbf{Train}}
 & \multicolumn{2}{c}{\textbf{Test}}\\

 & Arr & SR
 & Arr & SR
 & Arr & SR
 & Arr & SR 
 \\
 
\hline 
 Inspire & 0.62 & 0.88 & 0.41 & 0.44 & 0.52 & 0.26 & 0.22 & 0.00\\
 

 Ours w/o planner. & 0.44 & 0.88  & 0.20  & 0.19  & 0.05  & 0.22\\
 \textbf{Ours} &\textbf{0.99}  & \textbf{0.91}  & \textbf{0.81}  & \textbf{0.72}  & \textbf{0.75}  & \textbf{0.89}\\
\hline

\end{tabular}
}
\label{tab:base_exp}
\end{center}
\end{table}

==> tabs/real_and_analysis.tex <==
\begin{figure}
\centering
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{rebuttal_pics/DiffHeightObj.png}
    \caption{statistic analysis}
    \label{fig:re_analysis}
  \end{minipage}
\hfill

\begin{minipage}{0.48\textwidth}

\caption{Results for the real-world experiments}

\centering
\label{tab:realworld}
\setlength{\tabcolsep}{2.0mm}
\begin{tabular}{l|cccccc}

\toprule
& box-w1 & box-w2  & box-w3 & bag-w1 & container & handbag\\

\midrule
Wall  & 6/10 & 8/10 &  7/10 & 9/10 & 9/10 & 9/10 \\

\toprule
 & box-e1 & box-e2  & bag-e1 & bag-e2 & plate & handbag\\

\midrule
Edge    & 10/10   & 7/10       &  10/10 & 8/10 & 5/10 & 9/10  \\



\bottomrule

\end{tabular}
% \vspace{5pt}

\end{minipage}

\end{figure}

==> tabs/task_general.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!t]
\caption{
   Performance of objects with varying height in Wall and Edge task. 
   % , and the necessities of different components of our method.
   }
\label{tab:general}
\centering
\setlength{\tabcolsep}{6pt}
\small
\begin{tabular}{l|ccc|ccc}

\toprule
 & \multicolumn{3}{c|}{Wall} & \multicolumn{3}{c}{Edge} \\

\midrule
Object Height
 & TTE & PTE & SR
 & TTE & PTE & SR 
 \\
\midrule
$\leq 3cm$ 
& 0.23  & 7.79  & 0.76  
& 4.20  & 16.21  & 0.28\\

$3 - 4cm$ 
& 0.21  & 8.76  & 0.77  
& 3.51  & 25.10  & 0.68\\

$4 - 5cm$ 
& 0.21  & 6.79  & 0.45 
& 3.46  & 27.12  & 0.85\\

$\geq 5cm$ 
& 0.20  & 9.28  & 0.43  
& 3.67  & 24.22  & 0.91\\

% Ours w/o JT. & 0.44 & 0.88  & 0.20  & 0.19  & 0.05  & 0.22\\	

\bottomrule	

\end{tabular}


\end{table}
